Geometry-Aware Feature Matching for Large-Scale Structure from Motion

Establishing consistent and dense correspondences across multiple images is crucial for Structure from Motion (SfM) systems. Significant view changes, such as air-to-ground with very sparse view overlap, pose an even greater challenge to the correspondence solvers. We present a novel optimization-based approach that significantly enhances existing feature matching methods by introducing geometry cues in addition to color cues. This helps fill gaps when there is less overlap in large-scale scenarios. Our method formulates geometric verification as an optimization problem, guiding feature matching within detector-free methods and using sparse correspondences from detector-based methods as anchor points. By enforcing geometric constraints via the Sampson Distance, our approach ensures that the denser correspondences from detector-free methods are geometrically consistent and more accurate. This hybrid strategy significantly improves correspondence density and accuracy, mitigates multi-view inconsistencies, and leads to notable advancements in camera pose accuracy and point cloud density. It outperforms state-of-the-art feature matching methods on benchmark datasets and enables feature matching in challenging extreme large-scale settings.

==> sec/X_figure.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=1\linewidth]{imgs/IMC_ALL.pdf}
    \caption{\textbf{Qualitative results}. Our method is qualitatively compared with other feature matching methods on IMC 2021 Phototourism Dataset\cite{Jin2020}. Green cameras have less than 3\degree absolute pose error, while red cameras have an error larger than 3\degree.}
    \label{fig:imc_rec}
\end{figure*}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=1\linewidth]{imgs/ScanNet_1.pdf}
    \caption{\textbf{Qualitative results}. Our method is qualitatively compared with other feature matching methods on ScanNet Dataset\cite{dai2017scannet}. Green cameras have less than 3\degree absolute pose error, while red cameras have an error larger than 3\degree.}
    \label{fig:imc_rec}
\end{figure*}


\begin{figure*}[!ht]
    \centering
    \includegraphics[width=1\linewidth]{imgs/ScanNet_2.pdf}
    \caption{\textbf{Qualitative results}. Our method is qualitatively compared with other feature matching methods on ScanNet Dataset\cite{dai2017scannet}. Green cameras have less than 3\degree absolute pose error, while red cameras have an error larger than 3\degree.}
    \label{fig:imc_rec}
\end{figure*}


\begin{figure*}[!ht]
    \centering
    \includegraphics[scale=0.6]{imgs/cross_view.pdf}
    \caption{\textbf{Qualitative Matching Results on Collected Air-to-Ground Set 2}. Our method is able to find reliable matches for cross-view images.}
    \label{fig:cross_view}
\end{figure*}

\begin{figure*}[!ht]
    \centering
    \includegraphics[scale=0.5]{imgs/3dgs.png}
    \caption{\textbf{Qualitative Results of 3D gaussain splatting on Collected Air-to-Ground Set 2}. All 3D Gaussians are trained for 30,000 iterations. SIFT+NN fails in registering ground images with UAV images}
    \label{fig:3dgs}
\end{figure*}
